Level Truncation Approach to Open String Field Theory

Given a D-brane background in string theory (or equivalently boundary conditions in a two-dimensional conformal field theory), classical solutions of open string field theory equations of motion are conjectured to describe new D-brane backgrounds (boundary conditions). In this thesis, we study these solutions in bosonic open string field theory using the level truncation approach, which is a numerical approach where the string field is truncated to a finite number of degrees of freedom. We start with a review of the theoretical background and numerical methods which are needed in the level truncation approach and then we discuss solutions on several different backgrounds. First, we discuss universal solutions, which do not depend on the open string background, then we analyze solutions of the free boson theory compactified on a circle or on a torus, then marginal solutions in three different approaches and finally solutions in theories which include the A-series of Virasoro minimal models. In addition to known D-branes, we find so-called exotic solutions which potentially describe yet unknown boundary states. This paper is based on my doctoral thesis submitted to the Faculty of Mathematics and Physics at Charles University in Prague.

==> Thesis_bib.tex <==
\begin{thebibliography}{999}

%CFT

\bibitem{Runkel1}
  I.~Runkel,
  ``Boundary structure constants for the A series Virasoro minimal models,''
  Nucl.\ Phys.\ B {\bf 549} (1999) 563
  doi:10.1016/S0550-3213(99)00125-X
  [hep-th/9811178].

\bibitem{Runkel2}
  I.~Runkel,
  ``Structure constants for the D series Virasoro minimal models,''
  Nucl.\ Phys.\ B {\bf 579} (2000) 561
  doi:10.1016/S0550-3213(99)00707-5
  [hep-th/9908046].

\bibitem{Runkel3}
  I.~Runkel,
  ``Boundary problems in conformal field theory,'' PhD thesis,
    \url{https://www.math.uni-hamburg.de/home/runkel/PDF/phd.pdf}

\bibitem{DiFrancesco}
  P.~di~Francesco, P.~Mathieu and D.~Senechal,
  ``Conformal Field Theory,''
  Springer-Verlag (1997)

\bibitem{RecknagelSchomerus}
  A.~Recknagel and V.~Schomerus,
  ``Boundary Conformal Field Theory and the Worldsheet Approach to D-Branes,''
  Cambridge University Press (2013)

\bibitem{RecknagelSchomerusMarginal}
  A.~Recknagel and V.~Schomerus,
  ``Boundary deformation theory and moduli spaces of D-branes,''
  Nucl.\ Phys.\ B {\bf 545} (1999) 233
  doi:10.1016/S0550-3213(99)00060-7
  [hep-th/9811237].

\bibitem{Blumenhagen}
  R.~Blumenhagen and E.~Plauschinn,
  ``Introduction to Conformal Field Theory: With Applications to String Theory,''
  Springer-Verlag (2009)

\bibitem{LewellenSewing}
  D.~C.~Lewellen,
  ``Sewing constraints for conformal field theories on surfaces with boundaries,''
  Nucl.\ Phys.\ B {\bf 372} (1992) 654.
  doi:10.1016/0550-3213(92)90370-Q

\bibitem{MooreSeiberg}
  G.~Moore and N.~ Seiberg,
  ``Lectures on RCFT,``
  Physics, Geometry, and Topology, Plenum Press, New York, 1990.

\bibitem{BCRational}
  R.~E.~Behrend, P.~A.~Pearce, V.~B.~Petkova and J.~B.~Zuber,
  ``Boundary conditions in rational conformal field theories,''
  Nucl.\ Phys.\ B {\bf 570} (2000) 525
   [Nucl.\ Phys.\ B {\bf 579} (2000) 707]
  doi:10.1016/S0550-3213(99)00592-1, 10.1016/S0550-3213(00)00225-X
  [hep-th/9908036].

\bibitem{GaberdielBoson}
  M.~R.~Gaberdiel and A.~Recknagel,
  ``Conformal boundary states for free bosons and fermions,''
  JHEP {\bf 0111} (2001) 016
  doi:10.1088/1126-6708/2001/11/016
  [hep-th/0108238].

\bibitem{GaberdielBosonSU2}
  M.~R.~Gaberdiel, A.~Recknagel and G.~M.~T.~Watts,
  ``The Conformal boundary states for SU(2) at level 1,''
  Nucl.\ Phys.\ B {\bf 626} (2002) 344
  doi:10.1016/S0550-3213(02)00033-0
  [hep-th/0108102].

\bibitem{GaberdielBoundary}
  M.~R.~Gaberdiel,
  ``Boundary conformal field theory and D-branes,''
   \url{https://people.phys.ethz.ch/~mrg/CFT/Budapest.ps}

%Strings

\bibitem{Polchinski}
  J.~Polchinski,
  ``String theory. Vol. 1: An Introduction to the Bosonic String,''  Cambridge University Press (1998)

\bibitem{Polchinski2}
  J.~Polchinski,
  ``String theory. Vol. 2: Superstring Theory and Beyond,''  Cambridge University Press (1998)


\bibitem{BlumenhagenStringTheory}
R.~Blumenhagen, D.~L\"{u}st and S.~Theisen,
``Basic concepts of string theory,''
Springer (2013)


\bibitem{BeckerBeckerSchwarz}
K.~Becker, M.~Becker, J.~H.~Schwarz,
``String theory and M-theory: A modern introduction,''
Cambridge University Press (2006)

\bibitem{ZwiebachStrings}
 B.~Zwiebach,
``A First Course in String Theory,''
Cambridge University Press (2004)


\bibitem{GreenSchwarzWitten1}
 M.~B.~Green, J.~H.~Schwarz, E.~Witten,
``Superstring Theory: Volume 1, Introduction,''
Cambridge University Press (1987)

\bibitem{GreenSchwarzWitten2}
 M.~B.~Green, J.~H.~Schwarz, E.~Witten,
``Superstring Theory: Volume 2, Loop Amplitudes, Anomalies and Phenomenology,''
Cambridge University Press (1987)

\bibitem{Gepner}
  D.~Gepner,
  ``Space-Time Supersymmetry in Compactified String Theory and Superconformal Models,''
  Nucl.\ Phys.\ B {\bf 296} (1988) 757.
  doi:10.1016/0550-3213(88)90397-5

\bibitem{GepnerDbranes}
  A.~Recknagel and V.~Schomerus,
  ``D-branes in Gepner models,''
  Nucl.\ Phys.\ B {\bf 531} (1998) 185
  doi:10.1016/S0550-3213(98)00468-4
  [hep-th/9712186].

\bibitem{PolchinskiDbranes}
  J.~Polchinski,
  ``Tasi lectures on D-branes,''
  hep-th/9611050.

\bibitem{BachasDbranes}
  C.~P.~Bachas,
  ``Lectures on D-branes,''
  hep-th/9806199.

%homotopy

\bibitem{HomotopyAllowager}
  E.~L.~Allgower, K.~Georg,
  ``Introduction to Numerical Continuation Methods,''  Springer-Verlag Berlin Heidelberg (1990)

\bibitem{Homotopy1}
  ``The Principles of Polynomial Homotopy Continuation Methods,`` \url{http://homepages.math.uic.edu/~jan/srvart/node4.html}

\bibitem{HomotopyPHC}
  ``PHCpack: a general-purpose solver
for polynomial systems by homotopy continuation,`` \url{http://homepages.math.uic.edu/~jan/PHCpack/phcpack.html}

\bibitem{OpenMP}
  ``OpenMP,`` \url{https://www.openmp.org/}

%SFT

\bibitem{KudrnaThesis}
  M.~Kudrna,
  ``Level Truncation Approach to Open String Field Theory,''
  PhD thesis, \url{https://dspace.cuni.cz/bitstream/handle/20.500.11956/110558/140080054.pdf}

\bibitem{OhmoriReview}
  K.~Ohmori,
  ``A Review on tachyon condensation in open string field theories,''
  hep-th/0102085.

\bibitem{EllwoodHashimoto}
  A.~Hashimoto and N.~Itzhaki,
  ``Observables of string field theory,''
  JHEP {\bf 0201} (2002) 028
  doi:10.1088/1126-6708/2002/01/028
  [hep-th/0111092].

\bibitem{EllwoodInvariants}
  I.~Ellwood,
  ``The Closed string tadpole in open string field theory,''
  JHEP {\bf 0808} (2008) 063
  doi:10.1088/1126-6708/2008/08/063
  [arXiv:0804.1131 [hep-th]].

\bibitem{IshibashiEnergy}
  T.~Baba and N.~Ishibashi,
  ``Energy from the gauge invariant observables,''
  JHEP {\bf 1304} (2013) 050
  doi:10.1007/JHEP04(2013)050
  [arXiv:1208.6206 [hep-th]].

\bibitem{GaiottoRastelliSU11}
  D.~Gaiotto, L.~Rastelli, A.~Sen and B.~Zwiebach,
  ``Ghost structure and closed strings in vacuum string field theory,''
  Adv.\ Theor.\ Math.\ Phys.\  {\bf 6} (2003) 403
  [hep-th/0111129].

\bibitem{ZwiebachSU11}
  B.~Zwiebach,
  ``Trimming the tachyon string field with SU(1,1),''
  hep-th/0010190.

\bibitem{WittenSFT}
  E.~Witten,
  ``Noncommutative Geometry and String Field Theory,''
  Nucl.\ Phys.\ B {\bf 268} (1986) 253.
  doi:10.1016/0550-3213(86)90155-0

\bibitem{KOZ}
  M.~Kiermaier, Y.~Okawa and B.~Zwiebach,
  ``The boundary state from open string fields,''
  arXiv:0810.1737 [hep-th].

\bibitem{ConservationlawsArroyo}
  E.~A.~Arroyo,
  ``Conservation laws and tachyon potentials in the sliver frame,''
  JHEP {\bf 1106} (2011) 033
  doi:10.1007/JHEP06(2011)033
  [arXiv:1103.4830 [hep-th]].

\bibitem{SenBackground1}
  A.~Sen,
  ``On the Background Independence of String Field Theory,''
  Nucl.\ Phys.\ B {\bf 345} (1990) 551.
  doi:10.1016/0550-3213(90)90400-8

\bibitem{SenBackground2}
  A.~Sen,
  ``On the Background Independence of String Field Theory. 2. Analysis of On-shell S Matrix Elements,''
  Nucl.\ Phys.\ B {\bf 347} (1990) 270.
  doi:10.1016/0550-3213(90)90560-Z

\bibitem{SenBackground3}
  A.~Sen,
  ``On the background independence of string field theory. 3. Explicit Field redefinitions,''
  Nucl.\ Phys.\ B {\bf 391} (1993) 550
  doi:10.1016/0550-3213(93)90084-3
  [hep-th/9201041].

\bibitem{SenBackground4}
  A.~Sen and B.~Zwiebach,
  ``A Proof of local background independence of classical closed string field theory,''
  Nucl.\ Phys.\ B {\bf 414} (1994) 649
  doi:10.1016/0550-3213(94)90258-5
  [hep-th/9307088].

\bibitem{BerkovitsSuperstring}
  N.~Berkovits,
  ``Review of open superstring field theory,''
  hep-th/0105230.

\bibitem{ZwiebachTensor}
  M.~R.~Gaberdiel and B.~Zwiebach,
  ``Tensor constructions of open string theories. 1: Foundations,''
  Nucl.\ Phys.\ B {\bf 505} (1997) 569
  doi:10.1016/S0550-3213(97)00580-4
  [hep-th/9705038].

\bibitem{ThornSFT}
  C.~B.~Thorn,
  ``String Field Theory,''
  Phys.\ Rept.\  {\bf 175} (1989) 1.
  doi:10.1016/0370-1573(89)90015-X

\bibitem{ErlerLectures}
  T.~Erler,
  ``Four Lectures on Analytic Solutions in Open String Field Theory,''
  arXiv:1912.00521 [hep-th].

\bibitem{OkawaLectures}
  Y.~Okawa,
  ``Analytic methods in open string field theory,''
  Prog.\ Theor.\ Phys.\  {\bf 128} (2012) 1001.
  doi:10.1143/PTP.128.1001

\bibitem{MasudaAmplitudes}
  T.~Masuda and H.~Matsunaga,
  ``Deriving on-shell open string field amplitudes without using Feynman rules,''
  arXiv:1908.09784 [hep-th].

%TV numeric

\bibitem{SenUniversality}
  A.~Sen,
  ``Universality of the tachyon potential,''
  JHEP {\bf 9912} (1999) 027
  doi:10.1088/1126-6708/1999/12/027
  [hep-th/9911116].

\bibitem{TaylorZwiebach}
  W.~Taylor and B.~Zwiebach,
  ``D-branes, tachyons, and string field theory,''
  doi:10.1142/9789812702821\_0012
  hep-th/0311017.

\bibitem{RastelliZwiebach}
  L.~Rastelli and B.~Zwiebach,
  ``Tachyon potentials, star products and universality,''
  JHEP {\bf 0109} (2001) 038
  [hep-th/0006240].

\bibitem{SenZwiebachTV}
  A.~Sen and B.~Zwiebach,
  ``Tachyon condensation in string field theory,''
  JHEP {\bf 0003} (2000) 002
  doi:10.1088/1126-6708/2000/03/002
  [hep-th/9912249].

\bibitem{GaiottoRastelli}
  D.~Gaiotto and L.~Rastelli,
  ``Experimental string field theory,''
  JHEP {\bf 0308} (2003) 048
  doi:10.1088/1126-6708/2003/08/048
  [hep-th/0211012].

\bibitem{KishimotoTakahashi1}
  I.~Kishimoto and T.~Takahashi,
  ``Numerical Evaluation of Gauge Invariants for $a$-gauge Solutions in Open String Field Theory,''
  Prog.\ Theor.\ Phys.\  {\bf 121} (2009) 695
  doi:10.1143/PTP.121.695
  [arXiv:0902.0445 [hep-th]].

\bibitem{KishimotoTakahashi2}
  I.~Kishimoto and T.~Takahashi,
  ``Numerical Evaluation of Gauge Invariants for $a$-gauge Solutions in Open String Field Theory,''
  Theor.\ Math.\ Phys.\  {\bf 163} (2010) 710
  doi:10.1007/s11232-010-0054-y
  [arXiv:0910.3025 [hep-th]].

\bibitem{EllwoodTaylorCohomology}
  I.~Ellwood and W.~Taylor,
  ``Open string field theory without open strings,''
  Phys.\ Lett.\ B {\bf 512} (2001) 181
  doi:10.1016/S0370-2693(01)00673-6
  [hep-th/0103085].

\bibitem{EllwoodTaylorGauge}
  I.~Ellwood and W.~Taylor,
  ``Gauge invariance and tachyon condensation in open string field theory,''
  hep-th/0105156.

\bibitem{GiustoCohomology}
  S.~Giusto and C.~Imbimbo,
  ``Physical states at the tachyonic vacuum of open string field theory,''
  Nucl.\ Phys.\ B {\bf 677} (2004) 52
  doi:10.1016/j.nuclphysb.2003.10.037
  [hep-th/0309164].

\bibitem{ImbimboCohomology}
  C.~Imbimbo,
  ``The Spectrum of open string field theory at the stable tachyonic vacuum,''
  Nucl.\ Phys.\ B {\bf 770} (2007) 155
  doi:10.1016/j.nuclphysb.2007.01.035
  [hep-th/0611343].

\bibitem{HataTVSiegEq}
  H.~Hata and S.~Shinohara,
  ``BRST invariance of the nonperturbative vacuum in bosonic open string field theory,''
  JHEP {\bf 0009} (2000) 035
  doi:10.1088/1126-6708/2000/09/035
  [hep-th/0009105].

\bibitem{KosteleckySamuel}
  V.~A.~Kostelecky and S.~Samuel,
 ``On a Nonperturbative Vacuum for the Open Bosonic String,''
  Nucl.\ Phys.\ B {\bf 336} (1990) 263.
  doi:10.1016/0550-3213(90)90111-P

\bibitem{MoellerTaylorTV}
  N.~Moeller and W.~Taylor,
  ``Level truncation and the tachyon in open bosonic string field theory,''
  Nucl.\ Phys.\ B {\bf 583} (2000) 105
  doi:10.1016/S0550-3213(00)00293-5
  [hep-th/0002237].

\bibitem{Kishimoto26}
  I.~Kishimoto,
  ``On numerical solutions in open string field theory,''
  Prog.\ Theor.\ Phys.\ Suppl.\  {\bf 188} (2011) 155.
  doi:10.1143/PTPS.188.155

\bibitem{KudrnaUniversal}
  M.~Kudrna and M.~Schnabl,
  ``Universal Solutions in Open String Field Theory,''
  arXiv:1812.03221 [hep-th].

\bibitem{TaylorPerturbativeTV}
  W.~Taylor,
  ``A Perturbative analysis of tachyon condensation,''
  JHEP {\bf 0303} (2003) 029
  doi:10.1088/1126-6708/2003/03/029
  [hep-th/0208149].

\bibitem{SchnablQuadraticIdentities}
  M.~Schnabl,
  ``Constraints on the tachyon condensate from anomalous symmetries,''
  Phys.\ Lett.\ B {\bf 504} (2001) 61
  doi:10.1016/S0370-2693(01)00282-9
  [hep-th/0011238].

\bibitem{ArroyoSchablgauge}
  E.~A.~Arroyo, A.~Fernandes-Silva and R.~Szitas,
  ``Numerical solution of open string field theory in Schnabl gauge,''
  JHEP {\bf 1801} (2018) 007
  doi:10.1007/JHEP01(2018)007
  [arXiv:1707.09452 [hep-th]].

\bibitem{ArroyoKudrna}
  E.~Aldo Arroyo and M.~Kudrna,
  ``Numerical solution for tachyon vacuum in the Schnabl gauge,''
  JHEP {\bf 2002} (2020) 065
  doi:10.1007/JHEP02(2020)065
  [arXiv:1908.05330 [hep-th]].


\bibitem{KishimotoTTnum}
I.~Kishimoto and T.~Takahashi,
``Numerical twist-even SU(1,1)-singlet solutions in open string field theory around the identity-based solution,''
[arXiv:2011.08378 [hep-th]].

%boson numeric

\bibitem{MSZ lump}
  N.~Moeller, A.~Sen and B.~Zwiebach,
  ``D-branes as tachyon lumps in string field theory,''
  JHEP {\bf 0008} (2000) 039
  doi:10.1088/1126-6708/2000/08/039
  [hep-th/0005036].

\bibitem{KMS}
  M.~Kudrna, C.~Maccaferri and M.~Schnabl,
  ``Boundary State from Ellwood Invariants,''
  JHEP {\bf 1307} (2013) 033
  doi:10.1007/JHEP07(2013)033
  [arXiv:1207.4785 [hep-th]].

\bibitem{OhmoriLumps}
  K.~Ohmori,
  ``Survey of the tachyonic lump in bosonic string field theory,''
  JHEP {\bf 0108} (2001) 011
  doi:10.1088/1126-6708/2001/08/011
  [hep-th/0106068].

\bibitem{Lumps2DMoeller}
  N.~Moeller,
  ``Codimension two lump solutions in string field theory and tachyonic theories,''
  hep-th/0008101.

\bibitem{LumpsNDKoch}
  R.~de Mello Koch and J.~P.~Rodrigues,
  ``Lumps in level truncated open string field theory,''
  Phys.\ Lett.\ B {\bf 495} (2000) 237
  doi:10.1016/S0370-2693(00)01243-0
  [hep-th/0008053].

\bibitem{LumpsNDHarvey}
  J.~A.~Harvey and P.~Kraus,
  ``D-Branes as unstable lumps in bosonic open string field theory,''
  JHEP {\bf 0004} (2000) 012
  doi:10.1088/1126-6708/2000/04/012
  [hep-th/0002117].

\bibitem{LumpsKoch}
  R.~de Mello Koch, A.~Jevicki, M.~Mihailescu and R.~Tatar,
  ``Lumps and p-branes in open string field theory,''
  Phys.\ Lett.\ B {\bf 482} (2000) 249
  doi:10.1016/S0370-2693(00)00521-9
  [hep-th/0003031].

\bibitem{LumpSiegEq}
  P.~Mukhopadhyay and A.~Sen,
  ``Test of Siegel gauge for the lump solution,''
  JHEP {\bf 0102} (2001) 017
  doi:10.1088/1126-6708/2001/02/017
  [hep-th/0101014].

\bibitem{LumpsBeccaria}
  M.~Beccaria,
  ``D0-brane tension in string field theory,''
  JHEP {\bf 0509} (2005) 021
  doi:10.1088/1126-6708/2005/09/021
  [hep-th/0508090].

\bibitem{BeccariaConservation}
  M.~Beccaria and C.~Rampino,
  ``Level truncation and the quartic tachyon coupling,''
  JHEP {\bf 0310} (2003) 047
  doi:10.1088/1126-6708/2003/10/047
  [hep-th/0308059].

\bibitem{KudrnaVosmera}
  M.~Kudrna and J.~Vosmera,
  In preperation.

%Ising

\bibitem{Ising}
  M.~Kudrna, M.~Rapcak and M.~Schnabl,
  ``Ising model conformal boundary conditions from open string field theory,''
  arXiv:1401.7980 [hep-th].

\bibitem{OshikawaAffleckIsing}
  M.~Oshikawa and I.~Affleck,
  ``Boundary conformal field theory approach to the critical two-dimensional Ising model with a defect line,''
  Nucl.\ Phys.\ B {\bf 495} (1997) 533
  [cond-mat/9612187].

\bibitem{YangDoubleIsing}
  S.~-K.~Yang,
  ``Modular Invariant Partition Function Of The Ashkin-teller Model On The Critical Line And N=2 Superconformal Invariance,''
  Nucl.\ Phys.\ B {\bf 285} (1987) 183.

\bibitem{SchnablDefects}
  T.~Kojita, C.~Maccaferri, T.~Masuda and M.~Schnabl,
  ``Topological defects in open string field theory,''
  JHEP {\bf 1804} (2018) 057
  doi:10.1007/JHEP04(2018)057
  [arXiv:1612.01997 [hep-th]].

\bibitem{DefectsOSFT}
  K.~Budzik, M.~Rapcak and J.~M.~Rojas,
  ``Conformal Defects from String Field Theory,''
[arXiv:2009.06567 [hep-th]].

%marginal numeric

\bibitem{MarginalSen}
  A.~Sen and B.~Zwiebach,
  ``Large marginal deformations in string field theory,''
  JHEP {\bf 0010} (2000) 009
  [hep-th/0007153].

\bibitem{MarginalKMOSY}
  M.~Kudrna, T.~Masuda, Y.~Okawa, M.~Schnabl and K.~Yoshida,
  ``Gauge-invariant observables and marginal deformations in open string field theory,''
  JHEP {\bf 1301} (2013) 103
  doi:10.1007/JHEP01(2013)103
  [arXiv:1207.3335 [hep-th]].

\bibitem{MarginalTachyonKM}
  M.~Kudrna and C.~Maccaferri,
  ``BCFT moduli space in level truncation,''
  JHEP {\bf 1604} (2016) 057
  doi:10.1007/JHEP04(2016)057
  [arXiv:1601.04046 [hep-th]].

\bibitem{MarginalKishimotoNum}
  I.~Kishimoto and T.~Takahashi,
  ``Numerical Solutions of Open String Field Theory in Marginally Deformed Backgrounds,''
  PTEP {\bf 2013} (2013) no.9,  093B06
  doi:10.1093/ptep/ptt072
  [arXiv:1306.6532 [hep-th]].

%TV analytic

\bibitem{WedgeSchnabl}
  M.~Schnabl,
  ``Wedge states in string field theory,''
  JHEP {\bf 0301} (2003) 004
  doi:10.1088/1126-6708/2003/01/004
  [hep-th/0201095].

\bibitem{AnalyticSolutionSchnabl}
  M.~Schnabl,
  ``Analytic solution for tachyon condensation in open string field theory,''
  Adv.\ Theor.\ Math.\ Phys.\  {\bf 10} (2006) no.4,  433
  doi:10.4310/ATMP.2006.v10.n4.a1
  [hep-th/0511286].

\bibitem{AnalyticSolutionOkawa}
  Y.~Okawa,
  ``Comments on Schnabl's analytic solution for tachyon condensation in Witten's open string field theory,''
  JHEP {\bf 0604} (2006) 055
  doi:10.1088/1126-6708/2006/04/055
  [hep-th/0603159].

\bibitem{FuchsKroyterL0}
  E.~Fuchs and M.~Kroyter,
  ``Schnabl's L(0) operator in the continuous basis,''
  JHEP {\bf 0610} (2006) 067
  doi:10.1088/1126-6708/2006/10/067
  [hep-th/0605254].

\bibitem{ErlerKBC1}
  T.~Erler,
  ``Split String Formalism and the Closed String Vacuum,''
  JHEP {\bf 0705} (2007) 083
  doi:10.1088/1126-6708/2007/05/083
  [hep-th/0611200].

\bibitem{ErlerKBC2}
  T.~Erler,
  ``Split String Formalism and the Closed String Vacuum, II,''
  JHEP {\bf 0705} (2007) 084
  doi:10.1088/1126-6708/2007/05/084
  [hep-th/0612050].

\bibitem{SchnablLightningReview}
  M.~Schnabl,
  ``Algebraic solutions in Open String Field Theory - A Lightning Review,''
  Acta Polytechnica 50, no. 3 (2010) 102
  [arXiv:1004.4858 [hep-th]].

\bibitem{FuchsKroyterAnalytic}
  E.~Fuchs and M.~Kroyter,
  ``Analytical Solutions of Open String Field Theory,''
  Phys.\ Rept.\  {\bf 502} (2011) 89
  doi:10.1016/j.physrep.2011.01.003
  [arXiv:0807.4722 [hep-th]].




\bibitem{EllwoodTVCohomology}
  I.~Ellwood and M.~Schnabl,
  ``Proof of vanishing cohomology at the tachyon vacuum,''
  JHEP {\bf 0702} (2007) 096
  doi:10.1088/1126-6708/2007/02/096
  [hep-th/0606142].

\bibitem{TVAnalyticEquations}
  E.~Fuchs and M.~Kroyter,
  ``On the validity of the solution of string field theory,''
  JHEP {\bf 0605} (2006) 006
  doi:10.1088/1126-6708/2006/05/006
  [hep-th/0603195].

\bibitem{TVTakahashiNum}
  T.~Takahashi,
  ``Level truncation analysis of exact solutions in open string field theory,''
  JHEP {\bf 0801} (2008) 001
  doi:10.1088/1126-6708/2008/01/001
  [arXiv:0710.5358 [hep-th]].

\bibitem{TVArroyoPade}
  E.~A.~Arroyo,
  ``Cubic interaction term for Schnabl's solution using Pade approximants,''
  J.\ Phys.\ A {\bf 42} (2009) 375402
  doi:10.1088/1751-8113/42/37/375402
  [arXiv:0905.2014 [hep-th]].

\bibitem{SimpleAnalyticSolutionErlerSchnabl}
  T.~Erler and M.~Schnabl,
  ``A Simple Analytic Solution for Tachyon Condensation,''
  JHEP {\bf 0910} (2009) 066
  doi:10.1088/1126-6708/2009/10/066
  [arXiv:0906.0979 [hep-th]].

\bibitem{TVJokel}
  M.~Jokel,
  ``Real Tachyon Vacuum Solution without Square Roots,''
  arXiv:1704.02391 [hep-th].

\bibitem{TVArroyo}
  E.~A.~Arroyo,
  ``Comments on real tachyon vacuum solution without square roots,''
  JHEP {\bf 1801} (2018) 006
  doi:10.1007/JHEP01(2018)006
  [arXiv:1706.00336 [hep-th]].

\bibitem{Multibrane1}
  M.~Murata and M.~Schnabl,
  ``Multibrane Solutions in Open String Field Theory,''
  JHEP {\bf 1207} (2012) 063
  doi:10.1007/JHEP07(2012)063
  [arXiv:1112.0591 [hep-th]].

\bibitem{Multibrane2}
  M.~Murata and M.~Schnabl,
  ``On Multibrane Solutions in Open String Field Theory,''
  Prog.\ Theor.\ Phys.\ Suppl.\  {\bf 188} (2011) 50
  doi:10.1143/PTPS.188.50
  [arXiv:1103.1382 [hep-th]].

\bibitem{Multibrane3}
  H.~Hata and T.~Kojita,
  ``Winding Number in String Field Theory,''
  JHEP {\bf 1201} (2012) 088
  doi:10.1007/JHEP01(2012)088
  [arXiv:1111.2389 [hep-th]].

\bibitem{Multibrane4}
  H.~Hata and T.~Kojita,
  ``Singularities in K-space and Multi-brane Solutions in Cubic String Field Theory,''
  JHEP {\bf 1302} (2013) 065
  doi:10.1007/JHEP02(2013)065
  [arXiv:1209.4406 [hep-th]].

\bibitem{Multibrane5}
  H.~Hata and T.~Kojita,
  ``Inversion Symmetry of Gravitational Coupling in Cubic String Field Theory,''
  JHEP {\bf 1312} (2013) 019
  doi:10.1007/JHEP12(2013)019
  [arXiv:1307.6636 [hep-th]].

\bibitem{Multibrane6}
  H.~Hata,
  ``BV Analysis of Tachyon Fluctuation around Multi-brane Solutions in Cubic String Field Theory,''
  arXiv:1511.04187 [hep-th].

\bibitem{Multibrane7}
  T.~Masuda, T.~Noumi and D.~Takahashi,
  ``Constraints on a class of classical solutions in open string field theory,''
  JHEP {\bf 1210} (2012) 113
  doi:10.1007/JHEP10(2012)113
  [arXiv:1207.6220 [hep-th]].

\bibitem{Multibrane8}
  H.~Hata,
  ``Analytic Construction of Multi-brane Solutions in Cubic String Field Theory for Any Brane Number,''
  arXiv:1901.01681 [hep-th].

\bibitem{TVEllwoodTakahashi}
  T.~Kawano, I.~Kishimoto and T.~Takahashi,
  ``Gauge Invariant Overlaps for Classical Solutions in Open String Field Theory,''
  Nucl.\ Phys.\ B {\bf 803} (2008) 135
  doi:10.1016/j.nuclphysb.2008.05.025
  [arXiv:0804.1541 [hep-th]].

%marginal analytic

\bibitem{MarginalSchnablPert}
  M.~Schnabl,
  ``Comments on marginal deformations in open string field theory,''
  Phys.\ Lett.\ B {\bf 654} (2007) 194
  doi:10.1016/j.physletb.2007.08.023
  [hep-th/0701248 [HEP-TH]].

\bibitem{MarginalKiermaier}
  M.~Kiermaier, Y.~Okawa, L.~Rastelli and B.~Zwiebach,
  ``Analytic solutions for marginal deformations in open string field theory,''
  JHEP {\bf 0801} (2008) 028
  doi:10.1088/1126-6708/2008/01/028
  [hep-th/0701249 [HEP-TH]].

\bibitem{MarginalFuchs}
  E.~Fuchs, M.~Kroyter and R.~Potting,
  ``Marginal deformations in string field theory,''
  JHEP {\bf 0709} (2007) 101
  doi:10.1088/1126-6708/2007/09/101
  [arXiv:0704.2222 [hep-th]].

\bibitem{MarginalKiermaierOkawa}
  M.~Kiermaier and Y.~Okawa,
  ``Exact marginality in open string field theory: A General framework,''
  JHEP {\bf 0911} (2009) 041
  doi:10.1088/1126-6708/2009/11/041
  [arXiv:0707.4472 [hep-th]].

\bibitem{MarginalInatomi}
  S.~Inatomi, I.~Kishimoto and T.~Takahashi,
  ``Tachyon Vacuum of Bosonic Open String Field Theory in Marginally Deformed Backgrounds,''
  PTEP {\bf 2013} (2013) 023B02
  doi:10.1093/ptep/pts070
  [arXiv:1209.4712 [hep-th]].

\bibitem{MarginalMaccaferri}
  C.~Maccaferri,
  ``A simple solution for marginal deformations in open string field theory,''
  JHEP {\bf 1405} (2014) 004
  doi:10.1007/JHEP05(2014)004
  [arXiv:1402.3546 [hep-th]].

\bibitem{MarginalMaccaferriSchnabl}
  C.~Maccaferri and M.~Schnabl,
  ``Large BCFT moduli in open string field theory,''
  JHEP {\bf 1508} (2015) 149
  doi:10.1007/JHEP08(2015)149
  [arXiv:1506.03723 [hep-th]].

\bibitem{MarginalLaroccaMaccaferri}
  P.~V.~Larocca and C.~Maccaferri,
  ``BCFT and OSFT moduli: an exact perturbative comparison,''
  Eur.\ Phys.\ J.\ C {\bf 77} (2017) no.11,  806
  doi:10.1140/epjc/s10052-017-5379-3
  [arXiv:1702.06489 [hep-th]].

%boson analytic

\bibitem{LumpAnalytic1}
  L.~Bonora, C.~Maccaferri and D.~D.~Tolla,
  ``Relevant Deformations in Open String Field Theory: a Simple Solution for Lumps,''
  JHEP {\bf 1111} (2011) 107
  doi:10.1007/JHEP11(2011)107
  [arXiv:1009.4158 [hep-th]].

\bibitem{LumpAnalytic2}
  L.~Bonora, S.~Giaccari and D.~D.~Tolla,
  ``The energy of the analytic lump solution in SFT,''
  JHEP {\bf 1108} (2011) 158
   Erratum: [JHEP {\bf 1204} (2012) 001]
  doi:10.1007/JHEP08(2011)158, 10.1007/JHEP04(2012)001
  [arXiv:1105.5926 [hep-th]].

\bibitem{LumpAnalytic3}
  L.~Bonora, S.~Giaccari and D.~D.~Tolla,
  ``Analytic solutions for Dp branes in SFT,''
  JHEP {\bf 1112} (2011) 033
  doi:10.1007/JHEP12(2011)033
  [arXiv:1106.3914 [hep-th]].

\bibitem{LumpAnalytic4}
  L.~Bonora, S.~Giaccari and D.~D.~Tolla,
  ``Lump solutions in SFT. Complements,''
  arXiv:1109.4336 [hep-th].

\bibitem{LumpAnalytic5}
  T.~Erler and C.~Maccaferri,
  ``Comments on Lumps from RG flows,''
  JHEP {\bf 1111} (2011) 092
  doi:10.1007/JHEP11(2011)092
  [arXiv:1105.6057 [hep-th]].

\bibitem{ErlerMaccaferri}
  T.~Erler and C.~Maccaferri,
  ``String Field Theory Solution for Any Open String Background,''
  JHEP {\bf 1410} (2014) 029
  doi:10.1007/JHEP10(2014)029
  [arXiv:1406.3021 [hep-th]].

\bibitem{ErlerMaccaferri2}
  T.~Erler, C.~Maccaferri and R.~Noris,
  ``Taming boundary condition changing operator anomalies with the tachyon vacuum,''
  JHEP {\bf 1906} (2019) 027
  doi:10.1007/JHEP06(2019)027
  [arXiv:1901.08038 [hep-th]].

  \bibitem{ErlerMaccaferri3}
  T.~Erler and C.~Maccaferri,
  ``String field theory solution for any open string background. Part II,''
  JHEP {\bf 2001} (2020) 021
  doi:10.1007/JHEP01(2020)021
  [arXiv:1909.11675 [hep-th]].

\bibitem{VosmeraExotic}
  M.~Schnabl and J.~Vosmera,
  ``Gepner-like boundary states on $T^4$,''
  arXiv:1903.00487 [hep-th].

\bibitem{FluxAnalytic}
  N.~Ishibashi, I.~Kishimoto and T.~Takahashi,
  ``String field theory solution corresponding to constant background magnetic field,''
  PTEP {\bf 2017} (2017) no.1,  013B06
  doi:10.1093/ptep/ptw185
  [arXiv:1610.05911 [hep-th]].

\bibitem{FluxAnalytic2}
  N.~Ishibashi, I.~Kishimoto, T.~Masuda and T.~Takahashi,
  ``Vector profile and gauge invariant observables of string field theory solutions for constant magnetic field background,''
  JHEP {\bf 1805} (2018) 144
  doi:10.1007/JHEP05(2018)144
  [arXiv:1804.01284 [hep-th]].

\end{thebibliography}

%\bibitem{KishimotoCohomology}
%  I.~Kishimoto and T.~Takahashi,
%  ``Open string field theory around universal solutions,''
%  Prog.\ Theor.\ Phys.\  {\bf 108} (2002) 591
%  doi:10.1143/PTP.108.591
%  [hep-th/0205275]. 
